Hybrid Top-Down Global Causal Discovery with Local Search for Linear and Nonlinear Additive Noise Models

Learning the unique directed acyclic graph corresponding to an unknown causal model is a challenging task. Methods based on functional causal models can identify a unique graph, but either suffer from the curse of dimensionality or impose strong parametric assumptions. To address these challenges, we propose a novel hybrid approach for global causal discovery in observational data that leverages local causal substructures. We first present a topological sorting algorithm that leverages ancestral relationships in linear structural causal models to establish a compact top-down hierarchical ordering, encoding more causal information than linear orderings produced by existing methods. We demonstrate that this approach generalizes to nonlinear settings with arbitrary noise. We then introduce a nonparametric constraint-based algorithm that prunes spurious edges by searching for local conditioning sets, achieving greater accuracy than current methods. We provide theoretical guarantees for correctness and worst-case polynomial time complexities, with empirical validation on synthetic data.

==> figure_tex/figure_m_butterfly.tex <==
\begin{figure}[!h]
    \centering
\begin{tikzpicture}[scale=0.12]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [gray, fill=gray, fill opacity=0.1]  (30,-26.4) circle (3);
\draw (30,-26.4) node {$X$};
\draw [gray, fill=gray, fill opacity=0.1]  (44.7,-26.4) circle (3);
\draw (44.7,-26.4) node {$Y$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1]  (37.5,-19.8) circle (3);
\draw (37.5,-19.8) node {$Z_1$};
\draw [gray, fill=gray, fill opacity=0.1] (37.5,-10.5) circle (3);
\draw (37.5,-10.5) node {$B_3$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (30.6,-6) circle (3);
\draw (30.6,-6) node {$B_1$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (44.7,-6) circle (3);
\draw (44.7,-6) node {$B_2$};
\draw [gray, fill=gray, fill opacity=0.1]  (37.5,-41) circle (3);
\draw (37.5,-41) node {$Z_2$};
\draw [gray, fill=gray, fill opacity=0.1]  (37.5,-49.5) circle (3);
\draw (37.5,-49.5) node {$M_3$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1]  (44.7,-54.8) circle (3);
\draw (44.7,-54.8) node {$M_2$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (30,-54.8) circle (3);
\draw (30,-54.8) node {$M_1$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (55.2,-22.2) circle (3);
\draw (55.2,-22.2) node {$Z_{4}$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (20.7,-21.9) circle (3);
\draw (20.7,-21.9) node {$Z_{5}$};
\draw [gray, fill=gray, fill opacity=0.1] (55.2,-32.8) circle (3);
\draw (55.2,-32.8) node {$Z_6$};
\draw [gray, fill=gray, fill opacity=0.1] (20.7,-32.8) circle (3);
\draw (20.7,-32.8) node {$Z_7$};
\draw [gray, fill=gray, fill opacity=0.1] (37.5,-32.8) circle (3);
\draw (37.5,-32.8) node {$Z_3$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (55.2,-42.1) circle (3);
\draw (55.2,-42.1) node {$Z_8$};
%%%%%%%%
\draw [black,-{Latex[width=4pt]}] (33,-26.4) -- (41.7,-26.4);
\draw [black,-{Latex[width=4pt]}] (39.71,-21.83) -- (42.49,-24.37);
\draw [black,-{Latex[width=4pt]}] (35.25,-21.78) -- (32.25,-24.42);
\draw [black,-{Latex[width=4pt]}] (36.22,-13.21) -- (31.28,-23.69);
\draw [black,-{Latex[width=4pt]}] (38.74,-13.23) -- (43.46,-23.67);
\draw [black,-{Latex[width=4pt]}] (44.7,-9) -- (44.7,-23.4);
\draw [black,-{Latex[width=4pt]}] (30.51,-9) -- (30.09,-23.4);
\draw [black,-{Latex[width=4pt]}] (33.11,-7.64) -- (34.99,-8.86);
\draw [black,-{Latex[width=4pt]}] (42.16,-7.59) -- (40.04,-8.91);
\draw [black,-{Latex[width=4pt]}] (52.7,-23.9) -- (47.56,-25.51);
%\draw [black,-{Latex[width=4pt]}] (55.2,-19.2) -- (55.2,-16.6);
\draw [black,-{Latex[width=4pt]}] (23.4,-23.21) -- (27.3,-25.09);
%\draw [black,-{Latex[width=4pt]}] (20.7,-18.8) -- (20.7,-16.6);
\draw [black,-{Latex[width=4pt]}] (27.53,-28.1) -- (23.17,-31.1);
\draw [black,-{Latex[width=4pt]}] (47.26,-27.96) -- (52.64,-31.24);
\draw [black,-{Latex[width=4pt]}] (32.28,-28.35) -- (35.22,-30.85);
\draw [black,-{Latex[width=4pt]}] (39.74,-30.81) -- (42.46,-28.39);
\draw [black,-{Latex[width=4pt]}] (31.37,-29.07) -- (36.13,-38.33);
\draw [black,-{Latex[width=4pt]}] (43.37,-29.09) -- (38.83,-38.31);
\draw [black,-{Latex[width=4pt]}] (42.28,-53.02) -- (39.92,-51.28);
\draw [black,-{Latex[width=4pt]}] (32.45,-53.07) -- (35.05,-51.23);
%\draw [black,-{Latex[width=4pt]}] (52.48,-34.06) -- (40.22,-39.74);
\draw [black,-{Latex[width=4pt]}] (30,-51.8) -- (30,-29.4);
\draw [black,-{Latex[width=4pt]}] (44.7,-51.7) -- (44.7,-29.4);
\end{tikzpicture}
%%%%%%%%%%%%%
    \caption{A 16-node DAG with a butterfly structure and M-structure. Roots in red.}
    \label{fig:m_butterfly}
\end{figure}


==> figure_tex/figure_simple_tree.tex <==
\begin{figure}[!h]
    \centering
\begin{tikzpicture}[scale=0.12]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (23.8,-16.5) circle (3);
\draw (23.8,-16.5) node {$X_0$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (37.1,-16.5) circle (3);
\draw (37.1,-16.5) node {$X_1$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (50.3,-16.5) circle (3);
\draw (50.3,-16.5) node {$X_2$};
\draw [gray, fill=gray, fill opacity=0.1] (37.1,-28.6) circle (3);
\draw (37.1,-28.6) node {$X_3$};
\draw [gray, fill=gray, fill opacity=0.1] (37.1,-39.7) circle (3);
\draw (37.1,-39.7) node {$X_4$};
\draw [black,-{Latex[width=4pt]}] (26.02,-18.52) -- (34.88,-26.58);
\draw [black,-{Latex[width=4pt]}] (37.1,-19.5) -- (37.1,-25.6);
\draw [black,-{Latex[width=4pt]}] (37.1,-31.6) -- (37.1,-36.7);
\draw [black,-{Latex[width=4pt]}] (48.09,-18.53) -- (39.31,-26.57);
\end{tikzpicture}
    \caption{A simple tree structure with three roots (in red).}
    \label{fig:simple_tree}
\end{figure}

==> figure_tex/figure_square.tex <==
\begin{figure}[!h]
    \centering
\begin{tikzpicture}[scale=0.12]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (39.4,-16) circle (3);
\draw (39.4,-16) node {$X_1$};
\draw [gray, fill=gray, fill opacity=0.1] (22.9,-28.9) circle (3);
\draw (22.9,-28.9) node {$X_2$};
\draw [gray, fill=gray, fill opacity=0.1] (39.4,-28.9) circle (3);
\draw (39.4,-28.9) node {$X_3$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (22.9,-16) circle (3);
\draw (22.9,-16) node {$X_0$};
\draw [black,-{Latex[width=4pt]}] (25.26,-17.85) -- (37.04,-27.05);
\draw [black,-{Latex[width=4pt]}] (39.4,-19) -- (39.4,-25.9);
\draw [black,-{Latex[width=4pt]}] (22.9,-19) -- (22.9,-25.9);
\draw [black,-{Latex[width=4pt]}] (37.04,-17.85) -- (25.26,-27.05);
\end{tikzpicture}
%%%%%%
\hspace{10mm}
%%%%%%
\begin{tikzpicture}[scale=0.12]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (23.8,-16.5) circle (3);
\draw (23.8,-16.5) node {$X_0$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (37.1,-16.5) circle (3);
\draw (37.1,-16.5) node {$X_1$};
\draw [OrangeRed, fill=OrangeRed, fill opacity=0.1] (50.3,-16.5) circle (3);
\draw (50.3,-16.5) node {$X_2$};
\draw [gray, fill=gray, fill opacity=0.1] (37.1,-28.6) circle (3);
\draw (37.1,-28.6) node {$X_3$};
\draw [gray, fill=gray, fill opacity=0.1] (37.1,-39.7) circle (3);
\draw (37.1,-39.7) node {$X_4$};
\draw [black,-{Latex[width=4pt]}] (26.02,-18.52) -- (34.88,-26.58);
\draw [black,-{Latex[width=4pt]}] (37.1,-19.5) -- (37.1,-25.6);
\draw [black,-{Latex[width=4pt]}] (37.1,-31.6) -- (37.1,-36.7);
\draw [black,-{Latex[width=4pt]}] (48.09,-18.53) -- (39.31,-26.57);
\end{tikzpicture}
    \caption{A simple four-node DAG with two roots (left) and a simple tree with three roots (right). Roots in red.}
    \label{fig:simple_square}
\end{figure}

==> figure_tex/figure_triangles.tex <==
\begin{figure}[!h]
    \centering
%%%%%%%%%%%
%% CASE 1
%%%%%%%%%%%
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_1$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black,-{Latex[width=6pt]}] (47.41,-21.68) -- (43.79,-27.02);
%\fill [gray, fill=gray, fill opacity=0.2] (43.79,-27.02) -- (44.65,-26.64) -- (43.82,-26.08);
%% Z --> Y
\draw [black,-{Latex[width=6pt]}] (50.8,-21.67) -- (54.5,-27.03);
%\fill [gray, fill=gray, fill opacity=0.2] (54.5,-27.03) -- (54.45,-26.09) -- (53.63,-26.66);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\footnotesize \textbf{Case 1:} $Z$ is a confounder.};
\end{tikzpicture} \hspace{10mm} 
%%%%%%%%%%%
%% Case 2
%%%%%%%%%%%
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_2$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black,{Latex[width=6pt]}-] (47.41,-21.68) -- (43.79,-27.02);
%% Z --> Y
\draw [black,{Latex[width=6pt]}-] (50.8,-21.67) -- (54.5,-27.03);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\footnotesize \textbf{Case 2:} $Z$ is a collider.};
\end{tikzpicture}
%%%%%%%%%%%
%% CASE 3
%%%%%%%%%%%
\hspace{10mm}
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_3$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black, {Latex[width=6pt]}-] (47.41,-21.68) -- (43.79,-27.02);
%% Z --> Y
\draw [black,-{Latex[width=6pt]}] (50.8,-21.67) -- (54.5,-27.03);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\footnotesize \textbf{Case 3:} $Z$ is a mediator.};
\end{tikzpicture}
    \caption{Three possible causal triangles arise from the assumptions of this work: $Z$ is a confounder for $\{X,Y\}$, $Z$ is a collider for $\{X,Y\}$, and $Z$ is a mediator for $\{X,Y\}$.}
    \label{fig:triangles}
\end{figure}

%node[left,above,yshift=-2em,sloped]{$\alpha$} 

==> figure_tex/figure_triangles_coefficients.tex <==
\begin{figure}[!h]
    \centering
%%%%%%%%%%%
%% CASE 1
%%%%%%%%%%%
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_1$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black,-{Latex[width=6pt]}] (47.41,-21.68) -- node[left,above,xshift=-0.5em]{$b$} (43.79,-27.02);
%% Z --> Y
\draw [black,-{Latex[width=6pt]}] (50.8,-21.67) -- node[left,above,xshift=0.5em]{$c$} (54.5,-27.03);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- node[left,above,yshift=0.25em,sloped]{$a$}  (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\textbf{Case 1:} $\sigma_{xy} = a + bc$};
\end{tikzpicture} \hspace{10mm} 
%%%%%%%%%%%
%% Case 2
%%%%%%%%%%%
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_2$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black,{Latex[width=6pt]}-] (47.41,-21.68) -- node[left,above,xshift=-0.5em]{$b$} (43.79,-27.02);
%% Z --> Y
\draw [black,{Latex[width=6pt]}-] (50.8,-21.67) -- node[left,above,xshift=0.5em]{$c$} (54.5,-27.03);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- node[left,above,yshift=0.25em,sloped]{$a$} (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\textbf{Case 2:} $\sigma_{xy} = a$};
\end{tikzpicture}
%%%%%%%%%%%
%% CASE 3
%%%%%%%%%%%
\hspace{10mm}
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [WildStrawberry, fill=WildStrawberry, fill opacity=0.2] (49.1,-19.2) circle (3);
\draw (49.1,-19.2) node {$Z_3$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (42.1,-29.5) circle (3);
\draw (42.1,-29.5) node {$X$};
\draw [RoyalBlue, fill=RoyalBlue, fill opacity=0.2]  (56.2,-29.5) circle (3);
\draw (56.2,-29.5) node {$Y$};
%% Z --> X
\draw [black, {Latex[width=6pt]}-] (47.41,-21.68) -- node[left,above,xshift=-0.5em]{$b$} (43.79,-27.02);
%% Z --> Y
\draw [black,-{Latex[width=6pt]}] (50.8,-21.67) -- node[left,above,xshift=0.5em]{$c$} (54.5,-27.03);
%% X --> Y
\draw [black,-{Latex[width=6pt]}] (45.2,-29.5) -- node[left,above,yshift=0.25em,sloped]{$a$} (53.2,-29.5);
\draw [white,decorate,decoration={brace,amplitude=10pt,mirror}] (42.1,-35.5) -- (56.2,-35.5) node[black,midway,yshift=-0.1cm]{\textbf{Case 3:} $\sigma_{xy} = a + bc$};
\end{tikzpicture}
    \caption{Causal triangles with path coefficients.}
    \label{fig:triangles}
\end{figure}

